H$_2$ formation on interstellar dust grains: the viewpoints of theory, experiments, models and observations

Molecular hydrogen is the most abundant molecule in the universe. It is the first one to form and survive photo-dissociation in tenuous environments. Its formation involves catalytic reactions on the surface of interstellar grains. The micro-physics of the formation process has been investigated intensively in the last 20 years, in parallel of new astrophysical observational and modeling progresses. In the perspectives of the probable revolution brought by the future satellite JWST, this article has been written to present what we think we know about the H$_2$ formation in a variety of interstellar environments.

==> answer_to_the_referee.tex <==
Comments from the editors and reviewers:
-Reviewer 1

COMMENT 1: This manuscript gives comprehensive overview on the current view on H2 formation on interstellar dust. It covers a wide range of different aspects: theoretical, experimental, modelling and observational. It is in that aspect different from other recent reviews on H2 that typically covered only one or two of these aspects. The manuscript hence aims for a broad audience with different backgrounds. With that in mind, I sometimes miss some introduction and general context that would help people from different fields. Adding a figure of a typical spectrum (experimental or observational) would in some cases already help. See below for detailed comments.
ANSWER: WE ARE GRATEFUL TO THE REFEREE FOR HIS/HER DETAILED READING OF THE MANUSCRIPT AND THEIR APPRECIATION OF THE WIDE-RANGE OF OUR REVIEW. WE HAVE ANSWERED ALL THE REFEREE'S QUESTIONS/REMARKS AND INDICATED THE MODIFICATIONS IN BOLDFACE IN THE TEXT. THE DETAILED ANSWERS ARE GIVEN BELOW.  

COMMENT 2: page 2: I miss a reference to van de Hulst (1949) who, as far as I know, the first one to realize the importance of sur reactions.
ANSWER:  THE REFERENCE, ALTHOUGH DIFFICULT TO FIND, HAS BEEN ADDED TO THE INTRODUCTION. 

COMMENT 3: page 4 first paragraph:  g_u is the degeneracy of the upper level of the transition. 
ANSWER: WE HAVE CHANGED THIS AS SUGGESTED BY THE REFEREE.

COMMENT 4: page 4: "Three approaches are used" I only count two.
ANSWER: WE HAVE CHANGED THIS AS SUGGESTED BY THE REFEREE AND REFORMULATED THE SENTENCE.

COMMENT 5: section 2.1.4: it would help to already present Table 2 here and to include some of section 4.1. 
ANSWER: The paper was constructed in a way to expose general concepts at the beginning and then focus on the H2 chemistry in the different regions of the ISM in the second part of the paper. Moving section 4.1 and Table 2 to the beginning would dramatically change the balance of the paper and, in our opinion, it's logical flow. We however added a reference to section 4.1 in this section, so an interested reader knows where to find this information and that it is present later in the article. 

COMMENT 6: section 2.1.5: Add an observational spectrum. I miss some information about observations of atomic H, for instance in dark clouds (Goldsmith & Li); from this also information on H2 formation can be inferred.
ANSWER : WE HAVE ADDED A MENTION OF THE POSSIBILITY OF ESTIMATING THE MOLECULAR FRACTION INSIDE DENSE CLOUDS THROUGH HINSA OBSERVATIONS. IN ADDTION, THREE OBSERVATIONAL SPECTRA HAVE BEEN ADDED TO THE PAPER (FIGURES 4 TO 6) AS THE REFEREE SUGGESTS.

COMMENT 7: Section 2.2.1 + Fig 4: I do not really understand the distinction between "sticking" and "trapping" since only sticking is used in the remainder of the paper. An addition to figure 4 would help. Does sticking depend both on trapping and desorption?
ANSWER: WE HAVE ADDED A FEW WORDS TO THE TEXT TO CLARIFY THIS IMPORTANT POINT.

COMMENT 8: Page 11: The result by Katz et al gives only a lower limit to the H atom binding energy as higher values give degenerate results. The ratio of 0.7 is hence an upper limit.
ANSWER: THIS SENTENCE WAS REWORDED TO CLARIFY THIS POINT AS PER THE REVIEWER'S SUGGESTION. 

COMMENT 9: Page 11: An example TPD spectrum would be helpful for non-experimentalists
ANSWER: A FIGURE SHOWING TPD TRACES OF D2 FROM AN AMORPHOUS SILICATE SURFACE HAS BEEN ADDED (FIG 8).

COMMENT 10: Page 11: Goumans et al used an embedded cluster model where part of the surface was described by DFT and part by analytical potentials. The results should be very comparable with Garcia-Gil and Navarro-Ruiz since the most important part of the system is in all cases described by DFT.
ANSWER: These clarifications have now be included in the text.

COMMENT 11: Page 12: I miss results by Farebrother and Meijer et al on the E-R mechanism.
ANSWER: REFERENCES TO FAREBROTHER AND MEIJER HAVE BEEN ADDED.

COMMENT 12: Page 14: The work by Oba et al is on D + O2 instead of D2 + O2.
ANSWER: This typo has been corrected  and the text is now as the referee described. 

COMMENT 13: Page 14: "Molecular Dynamics calculations showed that the sticking coefficients of H atoms on ASW are near unity around 10 K" and "Some experiments indicate that the sticking coefficient is above 0.5 on an ASW sur at 10 K" is this sufficient agreement? I would like to see a bit more discussion on these two results, especially with this author list.
ANSWER: THIS PARAGRAPH HAS BEEN MODIFIED.

COMMENT 14: Page 15: A model is crucial in extracting information from experiments. A good example is the work of Katz et al versus Cazaux & Tielens or Cuppen & Herbst. I think the authors should stress this point more in their discussion. It is currently only mentioned in a small sentence, but it can have profound implications for the values that are finally chosen in Table 1.
ANSWER: TEXT INCORPORATING THIS SUGGESTION HAS BEEN ADDED TO  THE MANUSCRIPT. THE RELEVANT TEXT IS PLACED AT THE END OF SECTION 2.2.1.

COMMENT 15: Page 17: I miss citations to MC codes with can handle large networks by Chang et al and Vasyunin et al.
ANSWER: These references are now included in the text. 

COMMENT 16: Page 21: In what way is the sticking different than the transmission probability?
ANSWER:  THE STICKING PROBABILITY IS CALCULATED THEN THE PHONONS MODES ARE TAKEN INTO ACCOUNT IN THE DYNAMICS CALCULATIONS. WHILE, FOR THE CALCULATION OF TRANSMISSION PROBABILITY SUCH PHONON EFFECTS ARE NOT INCLUDED. THE TEXT HAS BEEN MODIFIED TO CLARIFY THIS POINT. 

COMMENT 17: Section 3.4 is very hard to read: characters B to H are not introduced. All abbreviations are simply listed. I recommend to make these footnotes of Table 1 and to treat the current footnotes in the same way (add categories I to M). The text of section 3.4 can then be used to introduce the different characters and abbreviations. The abbreviation NSC is not immediately clear. What is meant with energetic formation?
ANSWER: WE HAVE MODIFIED THE TABLE AND THE TEXT ACCORDING TO THE REFEREE'S SUGGESTION.

COMMENT 18: Page 28: Reactions with H2 do not only posses high barriers but are also exothermic in some cases (H2 + O -> H2O is a clear example) which effectively prevents tunneling through the barrier.
ANSWER: A sentence has been added to the text to mention this taking H2 + OH as an example.

COMMENT 19: Page 30: The formation of H2 has a clear impact on the main cooling mechanism in shocks (see for instance Cuppen et al)
ANSWER: The reference was added to the text.

Textual:
COMMENT 20: page 2:"In addition, over the last ten years great progresses" -> "progress"
ANSWER: WE HAVE CORRECTED THIS AS SUGGESTED BY THE REFEREE.

COMMENT 21: page 2: "so all the ro-vibrational transitions it undergoes are forbidden electric quadrupole transitions" -> "so all ro-vibrational transitions are forbidden electric quadrupole transitions"
ANSWER: WE HAVE CORRECTED THIS AS SUGGESTED BY THE REFEREE.

COMMENT 22: page 9: "there are usually just a handful of binding site that it is necessary to consider" -> "only a handful of binding sites need to be considered"
ANSWER: WE HAVE CORRECTED THIS AS SUGGESTED BY THE REFEREE.

COMMENT 23: page 9 and many other locations; objects do not have a genetive "graphite's hexagon" -> "hexagon of graphite"
ANSWER: WE HAVE CORRECTED THIS AS SUGGESTED BY THE REFEREE.

COMMENT 24: page 9 "Therefore" there is no causaul relationship.
ANSWER: THE SENTENCE BEGINNING "Therefore" HAS BEEN REMOVED. 

COMMENT 25: Page 17: (perhaps including... -> (possibly including ...
ANSWER: WE HAVE CORRECTED THIS AS SUGGESTED BY THE REFEREE.

COMMENT 26: Page 18: "mix up" -> "mix" ("mix up" means something like "mistake for")
ANSWER: WE HAVE CORRECTED THIS AS SUGGESTED BY THE REFEREE.

COMMENT 27: Page 18: to its connection with deuteration -> to their connection with deuteration
ANSWER: WE HAVE CORRECTED THIS AS SUGGESTED BY THE REFEREE.

COMMENT 28: Page 19: period after equation
ANSWER: WE HAVE CORRECTED THIS AS SUGGESTED BY THE REFEREE.

COMMENT 29: Page 19: sentence starting with "Due to the coupling" is impossible to read. Probably some brackets are missing. 
ANSWER: We have changed the sentence.

COMMENT 30: Page 20: "the sur temperature as also be a parameter"?????
ANSWER: WE CORRECTED THE TEXT TO READ "the surface temperature is also a parameter". 

COMMENT 31: Page 21: a spread of existing  -> a range of existing
ANSWER: WE HAVE CORRECTED THIS AS SUGGESTED BY THE REFEREE.

COMMENT 32: Page 23: D3: refrence -> reference
ANSWER: WE HAVE CORRECTED THIS AS SUGGESTED BY THE REFEREE.


